Fine-tune the pretrained ATST model for sound event detection

Sound event detection (SED) often suffers from the data deficiency problem. The recent baseline system in the DCASE2023 challenge task 4 leverages the large pretrained self-supervised learning (SelfSL) models to mitigate such restriction, where the pretrained models help to produce more discriminative features for SED. However, the pretrained models are regarded as a frozen feature extractor in the challenge baseline system and most of the challenge submissions, and fine-tuning of the pretrained models has been rarely studied. In this work, we study the fine-tuning method of the pretrained models for SED. We first introduce ATST-Frame, our newly proposed SelfSL model, to the SED system. ATST-Frame was especially designed for learning frame-level representations of audio signals and obtained state-of-the-art (SOTA) performances on a series of downstream tasks. We then propose a fine-tuning method for ATST-Frame using both (in-domain) unlabelled and labelled SED data. Our experiments show that, the proposed method overcomes the overfitting problem when fine-tuning the large pretrained network, and our SED system obtains new SOTA results of 0.587/0.812 PSDS1/PSDS2 scores on the DCASE challenge task 4 dataset.

==> trushbox.tex <==
% Three main approaches are proposed to address the data deficiency problem of SED: . Data augmentation aims at creating more samples/transformations from the given dataset. By audio warping \cite{park2019specaugment, nam2022filteraugment} or interpolation from different audio clips \cite{zhang2017mixup}, data augmentations could train the model with extra artificial samples and improve the transformation invariance of the model; SemiSL methods trains the model with low-cost but sufficient unlabelled data. The SemiSL-based SED systems mainly used the unlabelled audio clips by pseudo labeling \cite{tarvainen2017mean, verma2019interpolation} and consistency regularization \cite{koh2021sound, shao22rct}. The combination of these two strategies has shown promising results comparing with the supervised-only SED systems \cite{jiakai2018mean, zheng21skcrnn, nam22fdy, shao22rct}; And the parameter-sharing convolutional recurrent neural networks (CRNNs) \cite{jiakai2018mean, zheng21skcrnn, nam22fdy} are the most favorable models for SED, which alleviates the demand for training data and prevents the models from the overfitting problem under a limited amount of training data.


% Although the above three strategies mitigate the data deficiency problem for the SED systems, they still have some restrictions: the SemiSL methods assume that the unlabelled data shares an identical distribution with the labelled data, leaving tremendous out-of-distribution audio clips to be useless; The parameter-sharing CNNs mainly extract local spectral patterns, where the global patterns are ignored. To mitigate these restrictions, 


% The architecture of the our SED model is shown in Fig.~\ref{fig: arch}. We introduce the ATST-Frame to the SED system. ATST-Frame expresses SOTA performances on a series of downstream audio processing tasks. As a result, we regard ATST-Frame as a superior feature extractor which generates the linearly separable frame-level features for the SED. ATST-Frame uses a transformer encoder \cite{vaswani2017attention} as the feature extractor. Although the transformer model can learn long-term semantic information, ATST-Frame ignores the relationship among local time-spectral patches due to the inductive bias of the transformer model. Therefore, we keep the CRNN baseline model \cite{jiakai2018mean} unchanged and concatenate the 128-dimensional CNN features with the 768-dimensional ATST-Frame features, as a compensation of local information. Since the transformer model not only has a global view on the spectrograms but also generates shift-variant spectral features, there is no need for us to engineer the CNN module as in the recent CRNN systems \cite{zheng21skcrnn, nam22fdy}. An adaptive pooling layer is applied behind the ATST-Frame features to align the time-resolution of the ATST-Frame the same as that of the CNN module, followed by a 1-layer multilayer perceptron (MLP) to compress the 896-dimensional concatenated features to a dimension of 128. There are three modules in the proposed model: CNN, ATST-Frame and non-linear classifier modules. The CNN module consists of a 7-layer CNN with context gating activation layers \cite{jiakai2018mean}; The ATST-Frame part includes a frame-embedding projection layer and a 12-layer transformer encoder \cite{li2023self}; And the non-linear classifier module includes the merge layer, a 2-layer BiGRU plus a softmax-attention SED classifier \cite{jiakai2018mean}. 

% During training, instead of applying multiple data augmentations as in other SED systems \cite{shao22rct, li2023ast, Li2023panns}, we use only mixup \cite{zhang2017mixup} in training. ATST-Frame has a high resistance against the audio warping methods, considering that it has already been trained with heavily-warped audio clips in its pretext task \cite{li2023self}. And the warped samples would only affect the CNN features, leading the classifier to unexpectedly relies on the ATST-Frame features. 

% Formally, let the weak (clip-level) and strong (frame-level) predictions of the $i$th audio clip are 
% $\Hat{Y}_i^\text{m}$ and $\Hat{\mathbf{Y}}_i^\text{m}$, respectively. The superscript $\text{m} \in \{\text{s, t}\}$ stands for the student and teacher predictions, respectively. And $i \in N$ denotes the index of data sample among a total of $N$ data points. The two losses can be represented as 
% \begin{align}
% \mathcal{L}_{\text{MT}} = 
% \frac{1}{N} \sum^{N}_{i=1} \text{MSE}(\Hat{Y}_i^\text{s}, \Hat{Y}_i^\text{t}) +
% \frac{1}{N} \sum^{N}_{i=1} \text{MSE}(\Hat{\mathbf{Y}}_i^{\text{s}},\Hat{\mathbf{Y}}_i^{\text{t}}).
% \end{align}
% \begin{align}
% \mathcal{L}_{\text{ICT}} = \frac{1}{N}
% \sum^{N}_{i=1}(
% & \text{MSE}(\Hat{Y}_{i, j, \lambda}^{\text{s}},
% \lambda \Hat{Y}_i^{\text{t}} + (1 - \lambda) \Hat{Y}_j^{\text{t}}) + \notag\\
% & \text{MSE}(\Hat{\mathbf{Y}}_{i, j, \lambda}^{\text{s}}, \lambda \Hat{\mathbf{Y}}_i^{\text{t}} + (1 - \lambda)\Hat{\mathbf{Y}}_j^{\text{t}}),
% \end{align}
% where the subscript ${i, j, \lambda}$ denotes the audio clip indexes and mixup interpolation factor.


% $\mathcal{L_\text{BCE}}$, 
% \begin{align}
% \mathcal{L}_\text{BCE} = 
% \frac{1}{N^{\text{w}}} \sum^{N^{\text{w}}}_{i=1}\text{BCE}(\Hat{Y}_i^{\text{w}}, Y_i^{\text{w}}) +
% \frac{1}{N^{\text{s}}} \sum^{N^{\text{s}}}_{i=1} \text{BCE}(\Hat{\mathbf{Y}}_i^{\text{s}},\mathbf{Y}_i^{\text{s}}),
% \end{align}

% Data augmentation
% Audio warping methods \cite{park2019specaugment, koh2021sound, nam2022filteraugment} warp the audio spectrograms and labels with extra prior knowledge such that the transformed samples are regarded as novel input samples which distributed nearby the original samples. On the other hand, mixup \cite{zhang2017mixup} is proposed to upsample the datasets by the interpolations between two arbitrarily selected samples from the dataset; 

% Semi-supervised learning
% SemiSL methods seek to mine task-specific information from the unlabelled data. The unlabelled samples are less expensive to be obtained than supervised ones. E.g., in 2018 detection and classification acoustic scenes and events (DCASE) challenge, task 4 \footnote{dcase.community/challenge2018}, there were 14,412 unlabelled audio clips released for the domestic environment sound event detection (DESED) task \cite{turpault2019sound}. This number is approximately ten times greater than the amount of of the labelled data. SemiSL methods mainly leverage the unlabelled data by two strategies: pseudo labeling and consistency regularization. MeanTeacher \cite{tarvainen2017mean} ensembles the models in each training step by the exponential moving average (EMA) as a teacher model to provide pseudo labels for the unlabelled samples. interpolation consistency training (ICT) \cite{verma2019interpolation} further combines the mixup with pseudo labeling strategy, providing the interpolated pseudo labels for the mixed (interpolated) samples. The consistency regularization strategy constrains the model to give consistent outputs for the samples before and after data warping. The combination of these two strategies has shown promising improvements on the SemiSL-based SED \cite{jiakai2018mean, zheng21skcrnn, nam22fdy, shao22rct}; 

%Two types of pretrained models are used for the SED task: self-supervised  and supervised models. 
%SelfSL leverages task-agnostic pretext tasks to train representational strong feature extractors, which have shown superior performances on a series of audio processing downstream tasks \cite{li2022atst, Chen2023BEATs, li2023self}. 

% The novelties of our work are in three fold: 1) We introduce the cutting-edge SelfSL model, ATST-Frame \cite{li2023self}, to the SED system, which shows better SED performances than the BEATs features. 2) We propose a 2-stage finetuning strategy to finetune the ATST-Frame embedded in our SED system. In the stage 1, we freeze the ATST-Frame and train the CRNN model to cooperate with the ATST-Frame features. In the stage 2, we heavily weight on the unsupervised losses and rely on the pseudo labels of unlabelled data to finetune ATST-Frame. Such strategy avoids the finetuning from the overfitting problem and further promotes the SED system performances. 3) 

%The previous solutions of alleviating such problem mainly focus on data augmentation, semi-supervised learning and parameter-sharing networks. 
%However, these methods also bring some restrictions, by which the task-unrelated unsupervised data and large-scale neural networks cannot be used for SED. 


% E.g.,~in 2018 detection and classification acoustic scenes and events (DCASE) challenge, task 4\footnote{dcase.community/challenge2018}, there were 14,412 unlabelled audio clips released for the domestic environment sound event detection (DESED) task \cite{turpault2019sound}. This number is approximately ten times greater than the amount of of the labelled data.

 % Nevertheless, ATST-Frame is a large-scale model with over 80M parameters pretrained using over 2M audio clips, where the amount of supervised data in the DESED dataset \cite{turpault2019sound} is insufficient (5,048 real and 10,000 synthetic audio clips) to finetune of the ATST-Frame. Simply unfreezing the ATST-Frame in ATST-SED would result in an overfitting problem \cite{li2023self} where the ATST-Frame memorizes instead of learns from the training dataset. Furthermore, since the CNN and RNN classifier are not trained, the ATST-Frame is optimized to work in conjunction with the under-fitted modules. Such training objective may lead to the representation degeneration of the ATST-Frame features, resulting in poor performances on the SED. We propose to use the model initialization, heavily weighted unsupervised loss and data augmentations to tackle the above problems in fine-tuning. The flowchart of the proposed fine-tuning paradigm is shown in Fig.~\ref{fig: flowchart}. 

% Furthermore, since the CNN and RNN classifier are not trained, the ATST-Frame is optimized to work in conjunction with the under-fitted modules. Such training objective may lead to the representation degeneration of the ATST-Frame features, resulting in poor performances on the SED. 
% To avoid the representation degeneration, 
%we initialize our model by a pretrained ATST-SED system in the fine-tuning stage. This initial ATST-SED model is trained under the baseline training paradigm, whose 

% the CNN and non-linear classifier modules learn to work in conjunction with the frozen ATST-Frame features.
% With the initial model, the ATST-SED model is guaranteed to learn task-related knowledge in the fine-tuning. In fine-tuning, we first attempt to unfreeze the ATST-Frame only and freeze the rest part of the network. However, the ATST-Frame is fine-tuned to behave task-specifically for the SED task, where the task-unrelated spectral patterns are ignored in its generated features. To cooperate with such shifts of features, we also unfreeze all three modules when fine-tuning the ATST-SED model.

% In the proposed fine-tuning paradigm, we mainly rely on the unsupervised learning to overcome the overfitting problem, by fully leveraging the larger amount of unlabelled data (14,412 real audio clips) and adopting data augmentation to enrich the data diversity. For unsupervised learning, both MT and interpolation consistency training (ICT) losses are used.
% %For unsupervised learning, the MT loss is still used. 
% % ICT loss is widely used in the SemiSL based SED systems \cite{nam22fdy, zheng21skcrnn}. ICT can be regarded as the MT loss when the audio clips are mixed-up \cite{zhang2017mixup}. Instead of using the MT pseudo labels of the mixed samples, the ICT loss use the interpolated teacher pseudo labels of the two interpolated samples for the mixed samples. 
% %Therefore, when mixup is not activated, MT loss is used for unsupervised training, and the ICT loss is used otherwise. 

% The model is also trained with both the supervised BCE loss. and unsupervised MT loss as in the baseline system Eq.~(\ref{eq:loss}), but this time the weight $r$ for unsupervised MT loss is set much higher. 
% In addition, we apply data augmentation (mixup \cite{zhang2017mixup} and frequency warping \cite{li2023self} ) for one training batch with a probability of 0.5. 
% When data augmentation is applied, we use the interpolation consistency training (ICT) loss \cite{verma2019interpolation} to replace the regular MT loss, and a different weight (denoted as ${r}_{\text{ICT}}$) is used for unsupervised loss.
% ICT is an efficient SemiSL technique, and is widely used in SED systems \cite{nam22fdy, zheng21skcrnn}.

% As for the input of the ATST-Frame, the frame length is 64 ms with a hop length of 10 ms, and the dimension of LogMel feature is 64. Each 10-second sound clip is represented in the dimension of $626 \times 128$ for the CNN inputs and $1000 \times 64$ for the ATST-Frame. 

%Namely, the pretrained ATST-Frame model in ATST-SED and the pretrained BEATs model in BEATs-SED are trained with the same amount of training data. 
%Since BEATs-SED is trained with the original DESED dataset and does not utilize 3,470 real strongly-labelled audio clips from the AudioSet \cite{gemmeke2017audio}. 

% mixup is used for data augmentation, Instead of using the MT pseudo labels of the mixed samples, the ICT loss use the interpolated teacher pseudo labels of the two interpolated samples for the mixed samples. 
% the teacher pseudo labels are produced using the augmented data, while the student model still processes the original data. This type of MT loss is similar to the interpolation consistency training (ICT) loss \cite{verma2019interpolation} if mixup \cite{zhang2017mixup} is used for data augmentation. 
% . When data augmentation is applied, a different weight is used for unsupervised loss, denoted as $\tilde{r}$.
% Denoting $\gamma_{\text{MT}}$ as the weight for ICT loss, the unsupervised loss in the proposed fine-tuning method can be represented as
% \begin{align}
% \mathcal{L_\text{U}} = 
% \left\{
%     \begin{array}{lr}
%         \mathcal{L}_\text{MT}, & \text{mixup not used} \\
%         \gamma_{\text{ICT}} \mathcal{L}_\text{ICT}, & \text{otherwise}
%     \end{array}
% \right.
% \label{func: 1}
% \end{align}

% We notice that the amount of real audio clips in the unlabelled dataset (14,412) is approximately 3 times larger than that of the supervised dataset (5,048). 
% Since the total amount of the dataset is relatively large (approximately 30k), we suspect that the unsupervised loss might play a subtle role and that the abundant unlabelled samples are not fully utilized in the baseline training paradigm.
% Therefore, 
% \subsubsection{Data augmentations}
%We apply data augmentations to enrich the diversity of the training data. 
% As shown in Fig.~\ref{fig: flowchart},  mixup and frequency warping are applied for fine-tuning. Frequency warping was proposed in \cite{li2023self} for ATST-Frame pretraining. It  randomly stretches or squeezes the spectrogram in the frequency dimension, which is efficient to improve the frequency-transformation invariance for ATST-Frame. However, frequency warping is too difficult for the CNN module to learn, 
% % The CNN would extract meaningless or inconsistent patterns if the spectrograms are heavily squeezed or stretched under frequency warping. Therefore, 
% and we only apply it to the ATST-Frame inputs. 
% % Mixup is a widely used data augmentation method in SED. It randomly mixed (added) two audio clips as well as their corresponding labels by a random interpolation factor. 
% During fine-tuning, the mixup is used in conjunction with the unsupervised losses, which will be introduce in Sec.~\ref{sec: heavy_weight_unsup}. In each step of the finetuning, there is a 50\% chance to apply either of the augmentations.
